Engineering Crowdsourced Stream Processing Systems

A crowdsourced stream processing system (CSP) is a system that incorporates crowdsourced tasks in the processing of a data stream. This can be seen as enabling crowdsourcing work to be applied on a sample of large-scale data at high speed, or equivalently, enabling stream processing to employ human intelligence. It also leads to a substantial expansion of the capabilities of data processing systems. Engineering a CSP system requires the combination of human and machine computation elements. From a general systems theory perspective, this means taking into account inherited as well as emerging properties from both these elements. In this paper, we position CSP systems within a broader taxonomy, outline a series of design principles and evaluation metrics, present an extensible framework for their design, and describe several design patterns. We showcase the capabilities of CSP systems by performing a case study that applies our proposed framework to the design and analysis of a real system (AIDR) that classifies social media messages during time-critical crisis events. Results show that compared to a pure stream processing system, AIDR can achieve a higher data classification accuracy, while compared to a pure crowdsourcing solution, the system makes better use of human workers by requiring much less manual work effort.

==> removed.tex <==

\clearpage
\section*{REMOVED MATERIAL}

\spara{DBMS examples.}
specialized Data Stream Management Systems, for example, STREAM \cite{arasu2004stream}, Aurora \cite{carney2002monitoring}, TelegraphCQ \cite{chandrasekaran2003telegraphcq}.

Considering all the above mentioned dimensions, we believe that a data stream processing system that can collect, annotate and process data streams in real-time, must hold the following characteristics:

\begin{enumerate}
\item The system must be capable of handling continuous, high-speed incoming data streams that include both structured as well as unstructured data items.

\item The system should be flexible enough to be extensible and tailorable. This introduces the extendibility to hook any type of crowdsourcing platform, or to run the system using different types of processing techniques (i.e., clustering, classification, time-series analysis etc).

\item The system should support the processing of incoming data items in batch as well as real-time fashion.

\item The system should be capable of incorporating human-annotated inputs on data items to facilitate the underlaying techniques those require training data.

\item The system should be easily operable by non-programmers. Yet, being accessible for end-users is highly important as most of the times people who use these kinds of systems are domain-experts rather than IT experts.  
\end{enumerate}

Nevertheless, as of today we observed that all the required components of a system that we can call a "Data Stream Processing System" are independently available, however, to the best of our knowledge there exists no such system which encompasses all of the above mentioned characteristics under one roof or a system that provides a way to be extended.


platform for the \emphbf{acquisition, annotation}, and \emphbf{processing} of structured as well as unstructured data streams. The platform encompasses all the characteristics mention above, and mainly divided into three conceptual modules namely,  ``information collector", ``information annotator", and ``information processor". The whole platform is designed following the \emph{Separation of Concerns} design principal, that is, each of its modules (e.g., data collector, data processor and data annotator) completely designed to operate independently. A key aspect of the platform is its extensibility to any of the modules. Each module of the platform adopts an abstract model that exhibits enough expressive power to be able to easily extensible. 

\spara{Example stream data sources.}
Examples of such sources include, typically, traffic monitoring systems, environmental sensors, financial applications, and quite recently social networking websites (e.g., Twitter, Facebook, Google+, etc.), added to the stack. Each individual data item in the data streams can be a human-generated microblogging post on Twitter or Facebook, a web page click, a sensor reading, and so on.

\spara{Human intervention.}
This human intervention may take place through a crowdsoucing platforms, such as CrowdFlower\footnote{http://www.crowdflower.com/}, Amazon Mechanical Turk (AMT)\footnote{http://www.mturk.com/}, etc., or it can be provided by in-house experts.
%
For generality, we will assume it is crowdsourced as this is the ``difficult'' case. 
%
For generality, we will also consider arbitrary workflows in which manual and automatic processing steps are intermingled.

Figure \ref{fig:dsp-interactions} shows various interactions that could happen among different processing elements....

\begin{figure}[h!]
 \centering
    \includegraphics[width=\columnwidth]{figs/dsp-interactions}
  \caption{Various interaction patterns}
  \label{fig:dsp-interactions}
\end{figure} 

\spara{Knowledge-intensive crowdsourcing.}
For example, many knowledge-intensive applications (e.g. wiki article writing) work with non-decomposable tasks and sequential task handling (users write on one anothers' contributions, gradually ``building'' the article), with or without explicit collaboration. The input data is usually heterogeneous (e.g. wiki articles on different knowledge domains) and thus workers often need to access a large knowledge base (e.g. prior expertise, external web resources). The necessity to deal with heterogeneous data and the need to consult external sources usually mean that this type of crowdsourcing systems are high-latency ones.

\subsection{Inheritance from SPs and Cs}

Because of the application of automatic processing in some steps, CSPs can process more data stream elements than crowdsourcing systems (the latency of the human factor is reduced). Last, CSPs inherit from crowdsourcing systems the property of uncertainty (induced by the human element), which necessitates more robust and preventive (``plan B'') algorithms than those needed in SPs.

Reading the above, it becomes obvious that both the automatic and the human element bring along advantages and limitations to CSP systems.
%
In some cases, crowdsourced processing can be to some extent replaced by automatic processing (at a certain loss of quality). For instance, a face-detection algorithm with a lower-than-human recall can be used instead of a crowdsourcing task. In these cases, interesting trade-offs arise in the design.
%
For example, throughput can be increased and latency decreased by directing more items towards automatic processing instead of crowdsourcing, at the cost of a decrease in quality. The opposite may happen if we choose to process most or all the elements through crowdsourcing.


\section{Basic components}


\subsubsection{Definitions} \label{subsec:framework-preliminaries}

Before going into the details, in this section we first provide necessary concepts, definitions, and related terminologies, starting from our interpretation of a stream processing system:


\smallskip


\smallskip
\spara{Definition:} A {\em stream processing} system {\em ingests} data from various data sources, {\em processes} it in a flow according to a set of pre-compiled {\em processing rules} in a {\em timely manner}.
\smallskip

And, we define a crowd stream processing system as:

\smallskip
\spara{Definition:} A {\em crowdsourced stream processing} (CSP) system is a specialized class of {\em stream processing systems} (i.e., as defined above), that continuously ingests high-speed data produced by various types of data sources, processes it in a flow, additionally, allows {\em human-interventions}, and is capable to complete tasks in a {\em timely manner}.
\smallskip

\spara{Miscellaneous concepts and terminologies:}
We refer a {\em stream} as an unordered, unbounded, and possibly, unstructured infinite tokens called {\em data items}. We use term { \em Automatic Processing Element} (APE) where computer programs act as information processor, and, {\em Manual Processing Element} (MPE) where human-participation is involved for the processing of data items.

Thus, revising our definition of CSP system introducing our own terminologies ...

\section*{Framework}

\spara{From the application-level discussion.}

However, in addition to general, primitive types, the meta-model allows to use domain-specific types. We use term {\em composition} when multiple PEs connect and forms a particular topology.
%
A composition contains information of all the connections between multiple PEs, and it is the CSP system's responsibility to manage compositions. A connection between two processing elements can be of type {\em data flow} or {\em control flow}. Moreover, to fulfill different kinds of data communication needs, especially in data stream processing systems, the meta-model allows a data flow connection to behave as {\em buffered}, {\em distributed}, or as {\em broadcast} model.


%%%%%%%%%%%%%%%%

\subsection{Basic components}

\spara{Definition:} A {\em crowdsourced stream processing} (CSP) system is a connected directed graph consisting of a set of {\em Automatic Processing Elements} (APEs) and {\em Manual Processing Elements} (MPEs) connected together fulfilling a set of particular requirements in a {\em timely manner}.
\smallskip

Given these definitions, in this paper we provide necessary concepts, design principals, and formal models for the development of CSP systems through a model-drive approach. We first start with the definition of a general-purpose CSP framework, and second, we provide details on how we leverage the framework's capabilities to specialize it for a specific application domain (i.e., social media streams classification) that we present in the section 5.


\subsection{Model of a CSP system}\label{subsec:framework-pe}

To define the type of a CSP system, and in terms of modeling formalism, that what features the system should be able to support, it is necessary to define its meta-model that will also convey what expressive power it exhibits. As also briefly defined earlier this section, typically, crowdsourced stream processing systems comprised of a set of MPEs and APEs, which connect together to complete a job. They may require data flows or control flows, may require synchronization among various processing elements, and may allow concurrent access to data. The exact features of our generic framework is described by its {\em meta-model}, which is defined as below. 

\smallskip
\spara{Definition:} A {\em CSP system's meta-model} specifies a class of data stream processing systems, and thereby, the expressive power it exhibits, that is, the concepts, and composition capabilities, the underlying platform must know in order to support the development of that class of systems.
\smallskip

And, the processing elements in the system can be of type {\em information source}, {\em information processor}, or {\em information consumer}. 


In the next subsections we elaborate more on the concepts of APE, MPE and communication models. 

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=\columnwidth]{figs/dsp-topology}
%  \todo[ChaTo]{@Imran: I need to get your notation right in order to be able to graphically depict the design patterns.}
%  \caption{General Model of a CSP system}\label{fig:general-overview}
%\end{figure} 

\section*{Application: AIDR}

For the validation of our general-purpose framework, in the next section we present a hybrid data stream processing application that we implement following the design principals and meta-model described in this section.

Before presenting the details of application, we first present, in below, our motivations behind its development:

\spara{Motivation.} Twitter\footnote{http://twitter.com/} is a social media blogging platform, which has more than 500 million and growing users, that receives more than 340 million posts (i.e., tweets) daily \footnote{http://en.wikipedia.org/wiki/Twitter}.

We present AIDR (Artificial Intelligence for Disaster Response), a system designed and implemented following the design principals, specifications, and expressive power manifested by the general-purpose framework presented in the previous section. AIDR is a {\em crowdsourced stream processing system} and is comprised of a set of {\em automatic processing elements} (APE) and {\em manual processing elements} (MPE), that is, it leverages both human as well as computing powers. The core of the AIDR system

\section*{From the old introduction}

Typical cases in which human computation is required include:

\begin{itemize}
 \item As a final step, e.g. to review data that has been extracted automatically. This may be seen as a manual verification step, for instance, in systems for detecting attacks/intrusions in networks, for combating fraud in e-commerce, or for moderating user-generated content.
 \item As an initial step, e.g. to provide training examples to supervised machine learning algorithms.
 \item As an intermediate step, e.g. to provide labels that are then compared and validated automatically, and may generate new elements that require to be labeled.
\end{itemize}

\spara{Desiderata.}
A crowdsourced stream processing system should have, first, all the properties of a good stream processing system. For instance, one of the fundamental requirements of a stream processing system is to efficiently deal with high-speed data and processing workloads \cite{turaga2010design}. Moreover, to make actual processing more efficient, it is highly demanded to avoid unnecessary latencies such as network delays, persistence operations, etc. At peak times when incoming data-rate is high, an intended behavior is to drop or queue incoming data items depending on the situation. Moreover, processing strategies that cause processing elements to wait indefinitely are considered bad \cite{stonebraker20058}. 

In addition, a crowdsourced stream processing system should incorporate all the good properties of a crowdsourcing system. For instance, high-quality of crowdsourcing labels should be a priority, the acquisition of crowdsourcing labels should stay within a reasonable budget, and the crowdsourcing strategy should be re-active \cite{bozzon2013reactive}.




\begin{figure}[t]
\subfigure[Distributed model\label{fig:com-modality-distributed}]{\includegraphics[width=0.95\columnwidth]{figs/distributed-com}}
\subfigure[Broadcasted model\label{fig:com-modality-broadcasted}]{\includegraphics[width=0.95\columnwidth]{figs/broadcasting-com}}
\caption{Communication modalities}
\label{fig:communication-models}
\end{figure} 

%============

%Figure \ref{fig:dsp-collector-mm} shows the meta-model of the \emph{Information Collector} module of the system.
%\begin{figure}[tb]
% \centering
%    \includegraphics[width=\columnwidth]{figs/collector-metamodel}
%  \caption{Information Collector Meta-model}
%  \label{fig:dsp-collector-mm}
%\end{figure} 
%Specifically, we use Twitter as a streaming data source, that is, the system continuously collects and classifies tweets into multiple categories (e.g., donations, damage, causalities, etc.,) related to disasters. Moreover, the application uses crowdsourcing to fulfill the training data requirements. Before we proceed, let's consider the following scenario for better understanding.

%\spara{Scenario} Twitter\footnote{http://twitter.com/} is a social media blogging platform, which has more than 500 million and growing users, that receives more than 340 million posts (i.e., tweets) daily \footnote{http://en.wikipedia.org/wiki/Twitter}. During emergencies and disasters, Twitter plays an important role help disaster responders to quickly launch relief efforts. Let's say, we want to gather information about various kinds donations such as money, food, services, blood, etc. during a flood situation in a country. Considering the scale of information that flows on Twitter, it is challenging for disaster responders to investigate each individual tweet to look for desired information. For this purpose, we leverage different machine learning techniques (i.e., information classification, and extraction) to perform the job automatically. Moreover, we want human-workers to label a part of the incoming data to be used for the training purposes of the automatic techniques. 

%\begin{figure}[tb]
% \centering
%    \includegraphics[width=\columnwidth]{figs/scenario-model}
%  \caption{BPMN workflow modeling a tweets classification system}
%  \label{fig:scenario}
%\end{figure} 

%Figure \ref{fig:scenario} depicts a flow using BPMN notations comprised of various tasks connected together to server the required needs. The first task ``Get documents" is responsible to get tweets from Twitter against a user-defined query (i.e., tracking keywords, following specific Twitter users, etc.,) in real-time. The collected tweets are then consumed by the ``Feature extraction" and ``Prepare sample data" tasks. The ``Feature extraction" task extracts features (e.g., unigrams, bigrams) from the tweets, and the ``Prepare sample data" selects a small set of tweets to be passed to the ``Get human labeled data" task that is responsible for the human annotation of the tweets. A classifier is then trained using the annotated tweets, and gets triggered to start classifying incoming tweets in the ``Classify documents" tasks. From that point the classified tweets are consumed by consumers, and ``Prepare sample data" task again gets triggered to perform the human labelling until classifier reaches desired accuracy level.

%The requirements that we extract from the scenario are 1) we have to deal with a continuous high-speed Twitter stream that generates unstructured data, 2) the process involves both human as well as computers to complete the task, 3) in contrast to typical data stream processing flows, the specified flow additionally requires real-time human interventions to serve the need of training data. From the requirements we can clearly see that the traditional data processing systems are incapable to fulfill the demands of the specified and many other similar scenarios. To this end, in the next section, we present a conceptual framework of our proposed hybrid data processing system.


%--- role of human processing


%\subsubsection{By the number of passes over the streaming data}

%\note[ChaTo]{I think we can leave this out. The base case is one pass. We can speak about multiple passes in the conclusion or as an extension.}

%\spara{Single.} **TO ADD*


%\spara{Multiple.} **TO ADD**


%which is shown in the Figure~\ref{fig:eg-detect-verify} models human as post-processor (e.g., information verifier). This is when crowd verifies technology-generated output for validation and verification purposes. Although, in this case crowds are modeled in a serial way with technology, however, their response do not directly effect technology. The fourth interaction that we present, models human as a parallel processor, but this time technology is directly involved and effected by human responses. Figure 1.d depicts our fourth interaction showing crowds continuous involved providing labeled data on request form technology. 

%Complex architectures require a combination of parallel and serial connections.
%
%Figure~\ref{fig:eg-quality-task} presents humans act as a pre-processor (e.g., human as training data provider) in a serial way along with technology. That is, in order to enable technology to effectively start processing (e.g., supervised document classification), first crowds annotate and provide training data. In this case, as crowds and technology work in serial, so the technology waits for human-inputs to start processing. 

%In this section we look at existing crowdsourcing stream processing systems described in the literature, and try to describe some general classes.


\note[ChaTo]{Next paragraph clashes/repeats discussion already under design patterns.}

A final example is that of \emph{automatic quality assurance} CSPs, where an automatic process can ask for more labels until a certain quality criterion is satisfied (concisely summarized in the ``get another label'' notion by \citet{ipeirotis_2010_get_another_label}). The role of the automatic element here is therefore mainly that of aggregation, while, to facilitate this aggregation, the human element is mainly used in binary classification types of tasks. The composition of these systems is mainly parallel (many human elements working on the same task) and, in contrast with the examples described above, in this type of systems the passes over the same data stream part are multiple. Indicative examples of systems are those proposed by \cite{whang2013question} for entity resolution and by \citet{liu2012cdas} on data analytics (sentiment analysis and image tagging tasks).

...

when few human elements are involved (either in the number of people or in the number of times that people are requested to work on) then the CSP throughput is expected to increase and latency to reduce, as a result of the high involvement of the machine elements.
On the other hand, if no or very few automatic elements exist (e.g. used only to filter-out some very simple cases, but leaving the bulk of the work to humans) then latency may be high, but at the same time the performance in terms of quality is also expected to improve, as a result of the fact that more items are directly assessed by humans. 
Cost, as well as other elements are also expected to accordingly vary.
This trade-off between automatic and human processing elements is therefore expected to significantly affect the performance of the CSP and, as a direct result, its examination and balancing is something that the CSP designer need to carefully examine and balance. 

\spara{Context.} 
During emergencies and disasters (e.g., earthquakes, floods, hurricanes, etc.), social media can play an important role help disaster responders to quickly launch relief efforts to provide various kinds of services like food, shelter, water, money, medicine, etc. to effected people and ultimately can save hundreds of lives. Let's say, we want -- in real-time -- to gather information about various kinds humanitarian services people offer through their twitter posts such as money, food, services, blood, etc. during a flood situation in a country. 
%
Considering the scale of information that flows on Twitter, it is challenging for disaster responders to investigate each individual tweet in real-time to look for desired information. For this purpose, we want to leverage different machine learning techniques (i.e., information classification, and extraction) to perform the job automatically. Moreover, we want human-workers (i.e., volunteers and paid workers) to label a part of the incoming data to be used for the training purposes of machine learning algorithms. Above all, the whole process must be ingesting, processing and feeding consumers with credible information in {\em real-time} or with low latency.

\todo[ChaTo]{Edit the ``AIDR'' part.}

\spara{AIDR.}
The objective of AIDR is to classify messages that people post during disasters into a set of user-defined categories. For this purpose, the system continuously ingests data from Twitter, processes it (i.e., using machine learning classification techniques) and leverages human-participation (i.e., through crowdsourcing) when required, all in real-time. 

For the demonstration purposes, we designed AIDR specifically to operate on social media streams (i.e., Twitter in our case), that allowed us to showcase not all but most of the design patterns described in the section \ref{sec:desing-pattern}. Moreover, processing elements (PEs) in AIDR inherit all three classes specified by the processing elements meta-mode in the section \ref{sec:framework-pe}. That is, we have information sources, processors, and consumers. Information sources responsible of data ingestion from Twitter streaming API, processors perform data processing that is then consumed by the consumers. 

From the requirements specified in above, we can see that first of all we need  APE that continuously ingests data from Twitter streaming API against queries (i.e., set of hashtags, geographical locations, etc.) defined by disaster responders.  we intend AIDR system to be comprised of a set of information collectors, those can continuously ingest twitter posts against queries defined by disaster responders. Moreover, to effectively deal with multiple disasters at same time, we envision multiple information collectors running ingesting twitter data in real-time. This single requirement can have a huge impact on the underlying system design and consequently on overall performance. As typically during disaster tweets arrive at a very high-speed (e.g., during Sandy it was 2600 tweets/sec). So, a bad communication design between system's processing elements could cause serious performance issues. To this end, 

Moreover, the system intends to process collected data items, that is, the classification of data items to their appropriate categories. Typically a machine learning technique involves a number of pre-processing steps before effectively start its actual processing. For instance, this include data cleaning, feature extraction from the cleaned data, data sampling for annotation purposes, annotation of the data, and learning. Individual step in the process has its significance and hence required its proper adjustment in the flow following a appropriate design pattern and communication model presented in the section \ref{sec:framework-com}.


\begin{figure*}[th]
 \centering
    \includegraphics[width=\textwidth]{figs/dsp-detailed-model-v3}
  \caption{AIDR high-level architecture shows APEs and MPEs and their communications}
  \label{fig:csp-model}
\end{figure*}

\section*{Related work}

Real-time crowdsourcing, or {\em flash crowds} as named by \citet{kittur2013future}, are basically crowdsourcing stream processing systems that have low latency.

\citet{kulkami_2012_turkomatic} (Collaboratively crowdsourcing workflows with turkomatic) 

\spara{Real-time/ubiquituous crowdsourcing}

Crowd processing is a type of crowdsourcing involving the processing of a large amount of homogeneous external events/data elements~\cite{geiger_2011_crowdsourcing}.

Named entity annotation \cite{higgins2010mturk, finin2010annotating}, relevance evaluation \cite{alonso2008crowdsourcing}, seeking opinions \cite{mellebeek2010opinion}, and so on, are all examples of crowdsourcing tasks that require human-intervention when even sophisticated computer programs unable to produce good results. 

and \citet{franklin2011crowddb} describes an extension to SQL which involves crowdsourcing operations, and describes how to establish an efficient query plan, while 


\citet{mashhadi_2011_quality} (Quality Control for Real-time Ubiquitous Crowdsourcing) speaks of real-time events and dynamic crowds.

Moreover, to involve crowds for real-time work with tight completion-time requirements, such as \cite{bernstein2010soylent, bigham2010vizwiz}, poses serious challenges \cite{kittur2013future}.  

Real-time crowdsourcing, or {\em flash crowds} as named by \citet{kittur2013future}, are basically crowdsourcing stream processing systems that have low latency.

\citet{kulkami_2012_turkomatic} (Collaboratively crowdsourcing workflows with turkomatic) 

\citet{mashhadi_2011_quality} (Quality Control for Real-time Ubiquitous Crowdsourcing) speaks of real-time events and dynamic crowds.


(Towards Real-time Emergency Response using Crowd Supported Analysis of Social Media) describes a system in which there is an automatic selection of items to be annotated.

(TurKit: Tools for iterative tasks on mechanical turk) seems to be a paper about {\em pure crowdsourcing stream processing}, in which each step is crowdsourced.

\citet{fan2013hybrid} hybrid crowdsourcing system example.

\citet{whang2013question} seems to also be an example.

\citet{liu2012cdas} is another example for data cleaning.

\citet{wang_2013_transitive} (Leveraging Transitive Relations for Crowdsourced Joins) 



NOT USED LITERATURE

\spara{To check:}

\cite{dai_2013_pomdp} POMDP-based control of workflows for crowdsourcing, suggested by Ioanna.

\citet{shahabi_2013_spatial} (Towards a generic framework for trustworthy spatial crowdsourcing)

\citet{kittur_2011_crowdforge} (Crowdforge) Map-Reduce kind of architecture

\citet{bernstein_2011_twoseconds} (Crowds in two seconds: Enabling realtime crowd-powered interfaces)

\citet{kulkami_2012_turkomatic} (turkomatic) ... here the crowd can create a workflow between crowdsourced elements.

Check \url{http://scholar.google.com/scholar?q=crowdsourcing+process+data+control+flow+framework&btnG=&hl=en&as_sdt=0%2C5}

\tocite{Keep it simple: reward and task design in crowdsourcing} speaks about the effect of incentives and task complexity in accuracy (a dual task where workers must do two things yields lower accuracy than a singular task where workers are only asked to do one thing).

{\em Data stream management systems} include STREAM~\cite{arasu2004stream}, Aurora~\cite{carney2002monitoring}, NiagaraCQ~\cite{chen2000niagaracq}, and~TelegraphCQ \cite{chandrasekaran2003telegraphcq} among others. These systems are usually designed for application domains where persisting and querying the data is more important than being able to ingest and process data in real-time.
%, and often oriented to process data in batches as opposted to pure real-time stream processing systems that ingest and process continuous data streams in real-time. Moreover, the overall system performance in terms of throughput, and latency are not considered as crucial performance indicators in such systems. Most of the DSMSs allow writing and executing user-defined queries over data streams through their native query languages that are mostly of declarative nature except Aurora.


\section{Characterization of CSP}


% FOLLOW THE NOMENCLATURE OF "CROWDSOURCED PROCESSING ELEMENT" vs "AUTOMATIC PROCESSING ELEMENT"

%\note[ChaTo]{The next paragraph seems out of place.}
%\note[Yannick]{Right, but only the beginning of the paragraph, which should be put somewhere in the next paragraph describing CSPE functions. In the current paragraph, starting from "three broad classes of APE functions", this seems ok to me, because it describes the different functions that can have APE in the CSP.}
%WHAT


Human intelligence, provided by crowdsourcing workers, is used for tasks that can not be automated.
Among the tasks workers can execute we may find:  \emph{providing input} to other processing elements, \emph{correcting} an element's output, \emph{validating} that an  element performed as expected, and \emph{training} the automated processing elements so that they can learn to perform a task. 
%HOW
This leads to at least three broad classes of APE functions (see Fig.~\ref{fig:systemicCSP}): binary classification, n-ary classification, and open-ended contributions.
%
In \emph{binary classification}, workers are asked to give a ``yes/no'' answer to a given question: ``do these suspicious activities constitute an attack?'' \cite{debar2001aggregation}, ``does this entity correspond to this word in this context?''~\cite{demartini_2012_zencrowd}, ``do these two records correspond to the same person?''~\cite{whang2013question}.
%
In \emph{n-ary classification}, we can include
determining if a word in a sentence represents a person, a place, or an organization~\cite{finin2010annotating},
determining if an emergency-related tweet describes infrastructure damage, casualties, injuries, needs, etc.~\cite{imran2013extracting}, 
%determining which is the concept described by a column on a table on the web~\cite{fan2013hybrid},
determining which emotion corresponds to a tweet~\cite{liu2012cdas}, etc.
%performing relevance assessment ~\cite{alonso2008crowdsourcing},
%determining certain properties of a photo of a galaxy~\cite{kamar_2012_galaxyzoo}, etc.
%
In \emph{open-ended contributions}, workers are asked to perform an open-ended task such as:
``rewrite this sentence in a shorter way''~\cite{bernstein2010soylent},
%``describe how to sub-divide a complex task''~\cite{kulkami_2012_turkomatic},
``fill in the missing fields in this record''~\cite{franklin2011crowddb},
``make a drawing of an articulated figure''~\cite{demartini_2012_zencrowd} \inote{we should remove~\cite{demartini_2012_zencrowd}}, etc. 
This list is not comprehensive as new task types emerge as crowdsourcing systems (and CSPs) mature.

% (e.g. set ordering~\cite{mason_2010_financial}) 
end{comment}

\begin{comment}
\note[Ioanna]{We need to be careful with the following paragraph. We need to say where do these examples belong (from the above categories), or if they constitute a new category. For instance, relevance assessments or ordering of sets can be considered as n-ary classification, highlighting a sentence and tracing the boundaries of an object can be seen as binary (a region belongs or not to a person etc.) Drawing a figure is open-ended. Also, we have too many references for this sub-section perhaps.}

\note[ChaTo]{We have two options:

(a) We state that our list of "how" (binary classification, n-ary classification and open ended) is comprehensive, and hammer the other cases (sorting a list, selecting a sub-string, drawing) into the three classes.

(b) We state that our list of "how" is open-ended, and list different interaction modalities.

Personally I prefer (a), but I leave it to you Ioanna to decide.}

Other forms of interaction are possible: performing relevance assessments on a set of items~\cite{alonso2008crowdsourcing}, ordering a set of items~\cite{mason_2010_financial}, highlighting a part of a sentence~\cite{imran2013extracting}, tracing the boundaries of a person/object on an image~\cite{sorokin_2008_utility}, make a drawing of an articulated figure~\cite{demartini_2012_zencrowd}, etc.


%\todo[ChaTo]{We need a list, well-placed within the literature (i.e. with substantial overlaps with previous works), but focused on crowdsourced {\em stream processing}.}

%\spara{Confirm an automatic label.} ...

%\spara{Provide a training example for an automatic system.} ...
